A MeerKAT, e-MERLIN, H.E.S.S. and Swift search for persistent and transient emission associated with three localised FRBs

We report on a search for persistent radio emission from the one-off Fast Radio Burst (FRB) 20190714A, as well as from two repeating FRBs, 20190711A and 20171019A, using the MeerKAT radio telescope. For FRB 20171019A we also conducted simultaneous observations with the High Energy Stereoscopic System (H.E.S.S.) in very high energy gamma rays and searched for signals in the ultraviolet, optical, and X-ray bands. For this FRB, we obtain a UV flux upper limit of 1.39x10^-16 erg/cm^-2/s/Amstrong, X-ray limit of ~ 6.6x10^-14 erg/cm^-2/s and a limit on the very-high-energy gamma-ray flux (Phi) (E > 120 GeV) < 1.7 x 10^-12 erg/cm^-2/s. We obtain a radio upper limit of ~15 microJy/beam for persistent emission at the locations of both FRBs 20190711A and 20171019A, but detect diffuse radio emission with a peak brightness of ~53 microJy/beam associated with FRB 20190714A at z = 0.2365. This represents the first detection of the radio continuum emission potentially associated with the host (galaxy) of FRB 20190714A, and is only the third known FRB to have such an association. Given the possible association of a faint persistent source, FRB 20190714A may potentially be a repeating FRB whose age lies between that of FRB 20121102A and FRB 20180916A. A parallel search for repeat bursts from these FRBs revealed no new detections down to a fluence of 0.08 Jy ms for a 1 ms duration burst.

==> bibfile.tex <==
@ARTICLE{SCH+16,
   author = {{Spitler}, L.~G. and {Scholz}, P. and {Hessels}, J.~W.~T. and 
  {Bogdanov}, S. and {Brazier}, A. and {Camilo}, F. and {Chatterjee}, S. and 
  {Cordes}, J.~M. and {Crawford}, F. and {Deneva}, J. and {Ferdman}, R.~D. and 
  {Freire}, P.~C.~C. and {Kaspi}, V.~M. and {Lazarus}, P. and 
  {Lynch}, R. and {Madsen}, E.~C. and {McLaughlin}, M.~A. and 
  {Patel}, C. and {Ransom}, S.~M. and {Seymour}, A. and {Stairs}, I.~H. and 
  {Stappers}, B.~W. and {van Leeuwen}, J. and {Zhu}, W.~W.},
    title = "{A repeating fast radio burst}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1603.00581},
 primaryClass = "astro-ph.HE",
     year = 2016,
    month = mar,
   volume = 531,
    pages = {202-205},
      doi = {10.1038/nature17168},
   adsurl = {http://adsabs.harvard.edu/abs/2016Natur.531..202S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PHL+21,
       author = {{Petroff}, E. and {Hessels}, J.~W.~T. and {Lorimer}, D.~R.},
        title = "{Fast radio bursts at the dawn of the 2020s}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = jul,
          eid = {arXiv:2107.10113},
        pages = {arXiv:2107.10113},
archivePrefix = {arXiv},
       eprint = {2107.10113},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210710113P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CK+21,
       author = {{Caleb}, Manisha and {Keane}, Evan},
        title = "{A Decade and a Half of Fast Radio Burst Observations}",
      journal = {Universe},
         year = 2021,
        month = nov,
       volume = {7},
       number = {11},
        pages = {453},
          doi = {10.3390/universe7110453},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021Univ....7..453C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{10.1093/mnrasl/slu046,
    author = {Lyubarsky, Yuri},
    title = "{A model for fast extragalactic radio bursts}",
    journal = {MNRAS: Letters},
    volume = {442},
    number = {1},
    pages = {L9-L13},
    year = {2014},
    month = {04},
    abstract = "{Bursts of millisecond duration were recently discovered in the 1 GHz band. There is a strong evidence that they come from ∼1 Gpc distances, which implies extraordinary high-brightness temperature. I propose that these bursts could be attributed to synchrotron maser emission from relativistic, magnetized shocks. At the onset of the magnetar flare, a strongly magnetized pulse is formed, which propagates away through the relativistic magnetar wind and eventually reaches the nebula inflated by the wind within the surrounding medium. I show that the observed radio bursts could be generated at shocks formed via the interaction of the magnetic pulse with the plasma within the nebula. The model predicts strong millisecond bursts in the TeV band, which could be observed even from distant galaxies.}",
    issn = {1745-3925},
    doi = {10.1093/mnrasl/slu046},
    url = {https://doi.org/10.1093/mnrasl/slu046},
    eprint = {https://academic.oup.com/mnrasl/article-pdf/442/1/L9/9371140/slu046.pdf},
}


@ARTICLE{tavani2020xray,
       author = {{Tavani}, M. and {Casentini}, C. and {Ursi}, A. and {Verrecchia}, F. and {Addis}, A. and {Antonelli}, L.~A. and {Argan}, A. and {Barbiellini}, G. and {Baroncelli}, L. and {Bernardi}, G. and {Bianchi}, G. and {Bulgarelli}, A. and {Caraveo}, P. and {Cardillo}, M. and {Cattaneo}, P.~W. and {Chen}, A.~W. and {Costa}, E. and {Del Monte}, E. and {Di Cocco}, G. and {Di Persio}, G. and {Donnarumma}, I. and {Evangelista}, Y. and {Feroci}, M. and {Ferrari}, A. and {Fioretti}, V. and {Fuschino}, F. and {Galli}, M. and {Gianotti}, F. and {Giuliani}, A. and {Labanti}, C. and {Lazzarotto}, F. and {Lipari}, P. and {Longo}, F. and {Lucarelli}, F. and {Magro}, A. and {Marisaldi}, M. and {Mereghetti}, S. and {Morelli}, E. and {Morselli}, A. and {Naldi}, G. and {Pacciani}, L. and {Parmiggiani}, N. and {Paoletti}, F. and {Pellizzoni}, A. and {Perri}, M. and {Perotti}, F. and {Piano}, G. and {Picozza}, P. and {Pilia}, M. and {Pittori}, C. and {Puccetti}, S. and {Pupillo}, G. and {Rapisarda}, M. and {Rappoldi}, A. and {Rubini}, A. and {Setti}, G. and {Soffitta}, P. and {Trifoglio}, M. and {Trois}, A. and {Vercellone}, S. and {Vittorini}, V. and {Giommi}, P. and {D'Amico}, F.},
        title = "{An X-ray burst from a magnetar enlightening the mechanism of fast radio bursts}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
     volume = {5},
     pages = {401–407},
         year = 2021,
        month = feb,
          doi = {10.1038/s41550-020-01276-x},
archivePrefix = {arXiv},
       eprint = {2005.12164},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021NatAs.tmp...31T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Ridnaia:2021,
   title={A peculiar hard X-ray counterpart of a Galactic fast radio burst},
   ISSN={2397-3366},
   url={http://dx.doi.org/10.1038/s41550-020-01265-0},
   DOI={10.1038/s41550-020-01265-0},
   journal={Nature Astronomy},
   publisher={Springer Science and Business Media LLC},
   author={Ridnaia, A. and Svinkin, D. and Frederiks, D. and Bykov, A. and Popov, S. and Aptekar, R. and Golenetskii, S. and Lysenko, A. and Tsvetkova, A. and Ulanov, M. and et al.},
   year={2021},
   volume = {in press},
   month={Feb}
}

@article{INTEGRAL_BURST_A,
   title={INTEGRAL Discovery of a Burst with Associated Radio Emission from the Magnetar SGR 1935+2154},
   volume={898},
   ISSN={2041-8213},
   url={http://dx.doi.org/10.3847/2041-8213/aba2cf},
   DOI={10.3847/2041-8213/aba2cf},
   number={2},
   journal={ApJ},
   publisher={American Astronomical Society},
   author={Mereghetti, S. and Savchenko, V. and Ferrigno, C. and Götz, D. and Rigoselli, M. and Tiengo, A. and Bazzano, A. and Bozzo, E. and Coleiro, A. and Courvoisier, T. J.-L. and et al.},
   year={2020},
   month={Jul},
   pages={L29}
}

@misc{HXMT_Bursts,
    title={SGR J1935+2154 burst list},
    url={http://hxmten.ihep.ac.cn/bfy/331.jhtml},
    author = "{Insight-HXMT}",
    note = "{Accessed on January 2021}",
    year={2020}
}


@article{Brun_transient_tools,
    author = "Brun, F. and Piel, Q. and de Naurois, M. and Bernhard, S.",
    title = "{{Analysis methods to search for transient events in ground-based very high energy $\gamma$-ray astronomy}}",
    eprint = "2001.06084",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    doi = "10.1016/j.astropartphys.2020.102429",
    journal = "Astropart.Phys.",
    volume = "118",
    pages = "102429",
    year = "2020"
}

@ARTICLE{BDP+19,
       author = {{Bannister}, K.~W. and {Deller}, A.~T. and {Phillips}, C. and {Macquart}, J. -P. and {Prochaska}, J.~X. and {Tejos}, N. and {Ryder}, S.~D. and {Sadler}, E.~M. and {Shannon}, R.~M. and {Simha}, S. and {Day}, C.~K. and {McQuinn}, M. and {North-Hickey}, F.~O. and {Bhandari}, S. and {Arcus}, W.~R. and {Bennert}, V.~N. and {Burchett}, J. and {Bouwhuis}, M. and {Dodson}, R. and {Ekers}, R.~D. and {Farah}, W. and {Flynn}, C. and {James}, C.~W. and {Kerr}, M. and {Lenc}, E. and {Mahony}, E.~K. and {O'Meara}, J. and {Os{\l}owski}, S. and {Qiu}, H. and {Treu}, T. and {U}, V. and {Bateman}, T.~J. and {Bock}, D.~C. -J. and {Bolton}, R.~J. and {Brown}, A. and {Bunton}, J.~D. and {Chippendale}, A.~P. and {Cooray}, F.~R. and {Cornwell}, T. and {Gupta}, N. and {Hayman}, D.~B. and {Kesteven}, M. and {Koribalski}, B.~S. and {MacLeod}, A. and {McClure-Griffiths}, N.~M. and {Neuhold}, S. and {Norris}, R.~P. and {Pilawa}, M.~A. and {Qiao}, R. -Y. and {Reynolds}, J. and {Roxby}, D.~N. and {Shimwell}, T.~W. and {Voronkov}, M.~A. and {Wilson}, C.~D.},
        title = "{A single fast radio burst localized to a massive galaxy at cosmological distance}",
      journal = {Science},
     keywords = {ASTRONOMY, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2019,
        month = aug,
       volume = {365},
       number = {6453},
        pages = {565-570},
          doi = {10.1126/science.aaw5903},
archivePrefix = {arXiv},
       eprint = {1906.11476},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019Sci...365..565B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BSP+20,
       author = {{Bhandari}, Shivani and {Sadler}, Elaine M. and {Prochaska}, J. Xavier and
         {Simha}, Sunil and {Ryder}, Stuart D. and {Marnoch}, Lachlan and
         {Bannister}, Keith W. and {Macquart}, Jean-Pierre and {Flynn}, Chris and
         {Shannon}, Ryan M. and {Tejos}, Nicolas and {Corro-Guerra}, Felipe and
         {Day}, Cherie K. and {Deller}, Adam T. and {Ekers}, Ron and
         {Lopez}, Sebastian and {Mahony}, Elizabeth K. and
         {Nu{\~n}ez}, Consuelo and {Phillips}, Chris},
        title = "{The Host Galaxies and Progenitors of Fast Radio Bursts Localized with the Australian Square Kilometre Array Pathfinder}",
      journal = {\apjl},
     keywords = {Galaxies, Radio continuum emission, Radio bursts, Star formation, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = jun,
       volume = {895},
       number = {2},
          eid = {L37},
        pages = {L37},
          doi = {10.3847/2041-8213/ab672e},
archivePrefix = {arXiv},
       eprint = {2005.13160},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...895L..37B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{PMM+20,
       author = {{Prochaska}, J. Xavier and {Macquart}, Jean-Pierre and
         {McQuinn}, Matthew and {Simha}, Sunil and {Shannon}, Ryan M. and
         {Day}, Cherie K. and {Marnoch}, Lachlan and {Ryder}, Stuart and
         {Deller}, Adam and {Bannister}, Keith W. and {Bhandari}, Shivani and
         {Bordoloi}, Rongmon and {Bunton}, John and {Cho}, Hyerin and
         {Flynn}, Chris and {Mahony}, Elizabeth K. and {Phillips}, Chris and
         {Qiu}, Hao and {Tejos}, Nicolas},
        title = "{The low density and magnetization of a massive galaxy halo exposed by a fast radio burst}",
      journal = {Science},
     keywords = {ASTRONOMY, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = oct,
       volume = {366},
       number = {6462},
        pages = {231-234},
          doi = {10.1126/science.aay0073},
archivePrefix = {arXiv},
       eprint = {1909.11681},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019Sci...366..231P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{MPM+20,
       author = {{Macquart}, J. -P. and {Prochaska}, J.~X. and {McQuinn}, M. and
         {Bannister}, K.~W. and {Bhandari}, S. and {Day}, C.~K. and
         {Deller}, A.~T. and {Ekers}, R.~D. and {James}, C.~W. and
         {Marnoch}, L. and {Os{\l}owski}, S. and {Phillips}, C. and
         {Ryder}, S.~D. and {Scott}, D.~R. and {Shannon}, R.~M. and {Tejos}, N.},
        title = "{A census of baryons in the Universe from localized fast radio bursts}",
      journal = {\nat},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = may,
       volume = {581},
       number = {7809},
        pages = {391-395},
          doi = {10.1038/s41586-020-2300-2},
archivePrefix = {arXiv},
       eprint = {2005.13161},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020Natur.581..391M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MPH+17,
       author = {{Marcote}, B. and {Paragi}, Z. and {Hessels}, J.~W.~T. and
         {Keimpema}, A. and {van Langevelde}, H.~J. and {Huang}, Y. and
         {Bassa}, C.~G. and {Bogdanov}, S. and {Bower}, G.~C. and
         {Burke-Spolaor}, S. and {Butler}, B.~J. and {Campbell}, R.~M. and
         {Chatterjee}, S. and {Cordes}, J.~M. and {Demorest}, P. and
         {Garrett}, M.~A. and {Ghosh}, T. and {Kaspi}, V.~M. and {Law}, C.~J. and
         {Lazio}, T.~J.~W. and {McLaughlin}, M.~A. and {Ransom}, S.~M. and
         {Salter}, C.~J. and {Scholz}, P. and {Seymour}, A. and {Siemion}, A. and
         {Spitler}, L.~G. and {Tendulkar}, S.~P. and {Wharton}, R.~S.},
        title = "{The Repeating Fast Radio Burst FRB 121102 as Seen on Milliarcsecond Angular Scales}",
      journal = {\apjl},
     keywords = {radiation mechanisms: non-thermal, radio continuum: galaxies, techniques: high angular resolution, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2017,
        month = jan,
       volume = {834},
       number = {2},
          eid = {L8},
        pages = {L8},
          doi = {10.3847/2041-8213/834/2/L8},
archivePrefix = {arXiv},
       eprint = {1701.01099},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...834L...8M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{JOF+20,
       author = {{James}, C.~W. and {Os{\l}owski}, S. and {Flynn}, C. and {Kumar}, P. and
         {Bannister}, K. and {Bhandari}, S. and {Farah}, W. and {Kerr}, M. and
         {Lorimer}, D.~R. and {Macquart}, J. -P. and {Ng}, C. and
         {Phillips}, C. and {Price}, D.~C. and {Qiu}, H. and {Shannon}, R.~M. and
         {Spiewak}, R.},
        title = "{Which bright fast radio bursts repeat?}",
      journal = {\mnras},
     keywords = {methods: statistical, radio continuum: transients; fast radio bursts, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = may,
       volume = {495},
       number = {2},
        pages = {2416-2427},
          doi = {10.1093/mnras/staa1361},
archivePrefix = {arXiv},
       eprint = {1912.07847},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.495.2416J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CSR+19,
       author = {{Caleb}, M. and {Stappers}, B.~W. and {Rajwade}, K. and {Flynn}, C.},
        title = "{Are all fast radio bursts repeating sources?}",
      journal = {\mnras},
     keywords = {methods: data analysis, surveys, radio continuum: general, radio continuum: transients, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = apr,
       volume = {484},
       number = {4},
        pages = {5500-5508},
          doi = {10.1093/mnras/stz386},
archivePrefix = {arXiv},
       eprint = {1902.00272},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.484.5500C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{FAB+20,
       author = {{Fonseca}, E. and {Andersen}, B.~C. and {Bhardwaj}, M. and {Chawla}, P. and
         {Good}, D.~C. and {Josephy}, A. and {Kaspi}, V.~M. and {Masui}, K.~W. and
         {Mckinven}, R. and {Michilli}, D. and {Pleunis}, Z. and {Shin}, K. and
         {Tendulkar}, S.~P. and {Bandura}, K.~M. and {Boyle}, P.~J. and
         {Brar}, C. and {Cassanelli}, T. and {Cubranic}, D. and {Dobbs}, M. and
         {Dong}, F.~Q. and {Gaensler}, B.~M. and {Hinshaw}, G. and {Land
        ecker}, T.~L. and {Leung}, C. and {Li}, D.~Z. and {Lin}, H. -H. and
         {Mena-Parra}, J. and {Merryfield}, M. and {Naidu}, A. and {Ng}, C. and
         {Patel}, C. and {Pen}, U. and {Rafiei-Ravandi}, M. and {Rahman}, M. and
         {Ransom}, S.~M. and {Scholz}, P. and {Smith}, K.~M. and
         {Stairs}, I.~H. and {Vanderlinde}, K. and {Yadav}, P. and
         {Zwaniga}, A.~V.},
        title = "{Nine New Repeating Fast Radio Burst Sources from CHIME/FRB}",
      journal = {\apjl},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = mar,
       volume = {891},
       number = {1},
          eid = {L6},
        pages = {L6},
          doi = {10.3847/2041-8213/ab7208},
archivePrefix = {arXiv},
       eprint = {2001.03595},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...891L...6F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{CHIME_R2,
   author = {{The CHIME/FRB Collaboration}},
    title = "{A Second Source of Repeating Fast Radio Bursts}",
  journal = {arXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1901.04525},
 primaryClass = "astro-ph.HE",
 keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Instrumentation and Methods for Astrophysics},
     year = 2019,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2019arXiv190104525T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LGM+18,
       author = { C.~J. {Law} et al},
        title = "{Discovery of the Luminous, Decades-long, Extragalactic Radio Transient FIRST J141918.9+394036}",
      journal = {\apj},
     keywords = {catalogs, gamma-ray burst: general, radio continuum: general, stars: magnetars, surveys, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = Oct,
       volume = {866},
          eid = {L22},
        pages = {L22},
          doi = {10.3847/2041-8213/aae5f3},
archivePrefix = {arXiv},
       eprint = {1808.08964},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2018ApJ...866L..22L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{HF99,
       author = {{Hogg}, David W. and {Fruchter}, Andrew S.},
        title = "{The Faint-Galaxy Hosts of Gamma-Ray Bursts}",
      journal = {\apj},
     keywords = {GALAXIES: EVOLUTION, GAMMA RAYS: BURSTS, STARS: SUPERNOVAE: INDIVIDUAL: ALPHANUMERIC: SN 1998BW, X-RAYS: BURSTS, Galaxies: Evolution, Gamma Rays: Bursts, Stars: Supernovae: Individual: Alphanumeric: SN 1998bw, X-Rays: Bursts, Astrophysics},
         year = 1999,
        month = Jul,
       volume = {520},
        pages = {54-58},
          doi = {10.1086/307457},
archivePrefix = {arXiv},
       eprint = {astro-ph/9807262},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/1999ApJ...520...54H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{PBJ+16,
       author = {{Petroff}, E. and {Barr}, E.~D. and {Jameson}, A. and {Keane}, E.~F. and
         {Bailes}, M. and {Kramer}, M. and {Morello}, V. and {Tabbara}, D. and
         {van Straten}, W.},
        title = "{FRBCAT: The Fast Radio Burst Catalogue}",
      journal = {\pasa},
     keywords = {catalogs, methods: data analysis, telescopes, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = sep,
       volume = {33},
          eid = {e045},
        pages = {e045},
          doi = {10.1017/pasa.2016.35},
archivePrefix = {arXiv},
       eprint = {1601.03547},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016PASA...33...45P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{MSH+18,
   author = {D. {Michilli} et al},
    title = "{An extreme magneto-ionic environment associated with the fast radio burst source FRB 121102}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1801.03965},
 primaryClass = "astro-ph.HE",
 keywords = {Astrophysics - High Energy Astrophysical Phenomena},
     year = 2018,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv180103965M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CLW+17,
       author = {{Chatterjee}, S. and {Law}, C.~J. and {Wharton}, R.~S. and
         {Burke-Spolaor}, S. and {Hessels}, J.~W.~T. and {Bower}, G.~C. and
         {Cordes}, J.~M. and {Tendulkar}, S.~P. and {Bassa}, C.~G. and
         {Demorest}, P. and {Butler}, B.~J. and {Seymour}, A. and {Scholz}, P. and
         {Abruzzo}, M.~W. and {Bogdanov}, S. and {Kaspi}, V.~M. and
         {Keimpema}, A. and {Lazio}, T.~J.~W. and {Marcote}, B. and
         {McLaughlin}, M.~A. and {Paragi}, Z. and {Ransom}, S.~M. and
         {Rupen}, M. and {Spitler}, L.~G. and {van Langevelde}, H.~J.},
        title = "{A direct localization of a fast radio burst and its host}",
      journal = {\nat},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2017,
        month = jan,
       volume = {541},
       number = {7635},
        pages = {58-61},
          doi = {10.1038/nature20797},
archivePrefix = {arXiv},
       eprint = {1701.01098},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017Natur.541...58C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{LAB+17,
   author = { C.~J. {Law} et al},
    title = "{A Multi-telescope Campaign on FRB 121102: Implications for the FRB Population}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1705.07553},
 primaryClass = "astro-ph.HE",
 keywords = {radio continuum: stars, stars: neutron, supernovae: general, techniques: interferometric },
     year = 2017,
    month = nov,
   volume = 850,
      eid = {76},
    pages = {76},
      doi = {10.3847/1538-4357/aa9700},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...850...76L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{OYP18,
   author = {{Oppermann}, N. and {Yu}, H.-R. and {Pen}, U.-L.},
    title = "{On the non-Poissonian repetition pattern of FRB121102}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1705.04881},
 primaryClass = "astro-ph.HE",
 keywords = {methods: statistical, pulsars: general},
     year = 2018,
    month = apr,
   volume = 475,
    pages = {5109-5115},
      doi = {10.1093/mnras/sty004},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.475.5109O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{LBM+07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007Sci...318..777L},
	Archiveprefix = {arXiv},
	Author = {{Lorimer}, D.~R. and {Bailes}, M. and {McLaughlin}, M.~A. and {Narkevic}, D.~J. and {Crawford}, F.},
	Date-Added = {2014-07-11 00:57:57 +0000},
	Date-Modified = {2014-07-11 00:58:21 +0000},
	Doi = {10.1126/science.1147532},
	Eprint = {0709.4301},
	Journal = {\sci},
	Pages = {777-},
	Title = {A Bright Millisecond Radio Burst of Extragalactic Origin},
	Volume = {318},
	Year = {2007},
}

@ARTICLE{TSB+13,
       author = {{Thornton}, D. and {Stappers}, B. and {Bailes}, M. and {Barsdell}, B. and {Bates}, S. and {Bhat}, N.~D.~R. and {Burgay}, M. and {Burke-Spolaor}, S. and {Champion}, D.~J. and {Coster}, P. and {D'Amico}, N. and {Jameson}, A. and {Johnston}, S. and {Keith}, M. and {Kramer}, M. and {Levin}, L. and {Milia}, S. and {Ng}, C. and {Possenti}, A. and {van Straten}, W.},
        title = "{A Population of Fast Radio Bursts at Cosmological Distances}",
      journal = {Science},
     keywords = {ASTRONOMY Astronomy, Sociology, Physics, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2013,
        month = jul,
       volume = {341},
       number = {6141},
        pages = {53-56},
          doi = {10.1126/science.1236789},
archivePrefix = {arXiv},
       eprint = {1307.1628},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013Sci...341...53T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{SBC+17,
       author = {{Tendulkar}, S.~P. and {Bassa}, C.~G. and {Cordes}, J.~M. and
         {Bower}, G.~C. and {Law}, C.~J. and {Chatterjee}, S. and
         {Adams}, E.~A.~K. and {Bogdanov}, S. and {Burke-Spolaor}, S. and
         {Butler}, B.~J. and {Demorest}, P. and {Hessels}, J.~W.~T. and
         {Kaspi}, V.~M. and {Lazio}, T.~J.~W. and {Maddox}, N. and
         {Marcote}, B. and {McLaughlin}, M.~A. and {Paragi}, Z. and
         {Ransom}, S.~M. and {Scholz}, P. and {Seymour}, A. and
         {Spitler}, L.~G. and {van Langevelde}, H.~J. and {Wharton}, R.~S.},
        title = "{The Host Galaxy and Redshift of the Repeating Fast Radio Burst FRB 121102}",
      journal = {\apjl},
     keywords = {galaxies: distances and redshifts, galaxies: dwarf, galaxies: ISM, stars: magnetars, stars: neutron, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = jan,
       volume = {834},
       number = {2},
          eid = {L7},
        pages = {L7},
          doi = {10.3847/2041-8213/834/2/L7},
archivePrefix = {arXiv},
       eprint = {1701.01100},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...834L...7T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MNH+21,
       author = {{Marcote}, B. and {Nimmo}, K. and {Hessels}, J.~W.~T. and {Tendulkar}, S.~P. and {Bassa}, C.~G. and {Paragi}, Z. and {Keimpema}, A. and {Bhardwaj}, M. and {Karuppusamy}, R. and {Kaspi}, V.~M. and {Law}, C.~J. and {Michilli}, D. and {Aggarwal}, K. and {Andersen}, B. and {Archibald}, A.~M. and {Bandura}, K. and {Bower}, G.~C. and {Boyle}, P.~J. and {Brar}, C. and {Burke-Spolaor}, S. and {Butler}, B.~J. and {Cassanelli}, T. and {Chawla}, P. and {Demorest}, P. and {Dobbs}, M. and {Fonseca}, E. and {Giri}, U. and {Good}, D.~C. and {Gourdji}, K. and {Josephy}, A. and {Kirichenko}, A. Yu. and {Kirsten}, F. and {Landecker}, T.~L. and {Lang}, D. and {Lazio}, T.~J.~W. and {Li}, D.~Z. and {Lin}, H. -H. and {Linford}, J.~D. and {Masui}, K. and {Mena-Parra}, J. and {Naidu}, A. and {Ng}, C. and {Patel}, C. and {Pen}, U. -L. and {Pleunis}, Z. and {Rafiei-Ravandi}, M. and {Rahman}, M. and {Renard}, A. and {Scholz}, P. and {Siegel}, S.~R. and {Smith}, K.~M. and {Stairs}, I.~H. and {Vanderlinde}, K. and {Zwaniga}, A.~V.},
        title = "{A repeating fast radio burst source localized to a nearby spiral galaxy}",
      journal = {\nat},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = jan,
       volume = {577},
       number = {7789},
        pages = {190-194},
          doi = {10.1038/s41586-019-1866-z},
archivePrefix = {arXiv},
       eprint = {2001.02222},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020Natur.577..190M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{FDL+21,
       author = {{Fong}, Wen-fai and {Dong}, Yuxin and {Leja}, Joel and {Bhandari}, Shivani and {Day}, Cherie K. and {Deller}, Adam T. and {Kumar}, Pravir and {Prochaska}, J. Xavier and {Scott}, Danica R. and {Bannister}, Keith W. and {Eftekhari}, Tarraneh and {Gordon}, Alexa C. and {Heintz}, Kasper E. and {James}, Clancy W. and {Kilpatrick}, Charles D. and {Mahony}, Elizabeth K. and {Rouco Escorial}, Alicia and {Ryder}, Stuart D. and {Shannon}, Ryan M. and {Tejos}, Nicolas},
        title = "{Chronicling the Host Galaxy Properties of the Remarkable Repeating FRB 20201124A}",
      journal = {\apjl},
     keywords = {Radio transient sources, Radio bursts, Star formation, Stellar populations, Neutron stars, 2008, 1339, 1569, 1622, 1108, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = oct,
       volume = {919},
       number = {2},
          eid = {L23},
        pages = {L23},
          doi = {10.3847/2041-8213/ac242b},
archivePrefix = {arXiv},
       eprint = {2106.11993},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...919L..23F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{HMS+21,
       author = {{Hilmarsson}, G.~H. and {Michilli}, D. and {Spitler}, L.~G. and {Wharton}, R.~S. and {Demorest}, P. and {Desvignes}, G. and {Gourdji}, K. and {Hackstein}, S. and {Hessels}, J.~W.~T. and {Nimmo}, K. and {Seymour}, A.~D. and {Kramer}, M. and {Mckinven}, R.},
        title = "{Rotation Measure Evolution of the Repeating Fast Radio Burst Source FRB 121102}",
      journal = {\apjl},
     keywords = {Radio transient sources, Radio bursts, Radio astronomy, Time domain astronomy, Extragalactic magnetic fields, 2008, 1339, 1338, 2109, 507, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = feb,
       volume = {908},
       number = {1},
          eid = {L10},
        pages = {L10},
          doi = {10.3847/2041-8213/abdec0},
archivePrefix = {arXiv},
       eprint = {2009.12135},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...908L..10H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{MM18,
   author = {{Margalit}, B. and {Metzger}, B.~D.},
    title = "{A Concordance Picture of FRB 121102 as a Flaring Magnetar Embedded in a Magnetized Ion-Electron Wind Nebula}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1808.09969},
 primaryClass = "astro-ph.HE",
 keywords = {stars: magnetars },
     year = 2018,
    month = nov,
   volume = 868,
      eid = {L4},
    pages = {L4},
      doi = {10.3847/2041-8213/aaedad},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2018ApJ...868L...4M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CSA+20,
       author = {{Caleb}, M. and {Stappers}, B.~W. and {Abbott}, T.~D. and {Barr}, E.~D. and
         {Bezuidenhout}, M.~C. and {Buchner}, S.~J. and {Burgay}, M. and
         {Chen}, W. and {Cognard}, I. and {Driessen}, L.~N. and {Fender}, R. and
         {Hilmarsson}, G.~H. and {Hoang}, J. and {Horn}, D.~M. and
         {Jankowski}, F. and {Kramer}, M. and {Lorimer}, D.~R. and
         {Malenta}, M. and {Morello}, V. and {Pilia}, M. and {Platts}, E. and
         {Possenti}, A. and {Rajwade}, K.~M. and {Ridolfi}, A. and {Rhodes}, L. and
         {Sanidas}, S. and {Serylak}, M. and {Spitler}, L.~G. and
         {Townsend}, L.~J. and {Weltman}, A. and {Woudt}, P.~A. and {Wu}, J.},
        title = "{Simultaneous multi-telescope observations of FRB 121102}",
      journal = {\mnras},
     keywords = {transients: fast radio bursts, Surveys, Intergalactic medium, methods: data analysis, instrumentation: interferometers, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = jun,
       volume = {496},
       number = {4},
        pages = {4565-4573},
          doi = {10.1093/mnras/staa1791},
archivePrefix = {arXiv},
       eprint = {2006.08662},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.496.4565C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{WAXMAN17,
   author = {{Waxman}, E.},
    title = "{On the Origin of Fast Radio Bursts (FRBs)}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1703.06723},
 primaryClass = "astro-ph.HE",
 keywords = {masers, stars: neutron, supernovae: general},
     year = 2017,
    month = jun,
   volume = 842,
      eid = {34},
    pages = {34},
      doi = {10.3847/1538-4357/aa713e},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2017ApJ...842...34W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{YTK+18,
       author = {{Yamasaki}, Shotaro and {Totani}, Tomonori and {Kiuchi}, Kenta},
        title = "{Repeating and non-repeating fast radio bursts from binary neutron star mergers}",
      journal = {\pasj},
     keywords = {gravitational waves, radio continuum: general, stars: binaries: general, stars: neutron, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2018,
        month = jun,
       volume = {70},
       number = {3},
          eid = {39},
        pages = {39},
          doi = {10.1093/pasj/psy029},
archivePrefix = {arXiv},
       eprint = {1710.02302},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018PASJ...70...39Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PPP+18,
       author = {{Popov}, Sergei and {Postnov}, Konstantin and {Pshirkov}, Maxim},
        title = "{Fast radio bursts: Superpulsars, magnetars, or something else?}",
      journal = {International Journal of Modern Physics D},
     keywords = {Pulsars, magnetars, fast radio bursts, 95.85.Bh, 95.85.Fm, 97.60.Jd, Radio microwave, Submillimeter, Neutron stars, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = jan,
       volume = {27},
       number = {10},
          eid = {1844016},
        pages = {1844016},
          doi = {10.1142/S0218271818440169},
archivePrefix = {arXiv},
       eprint = {1801.00640},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018IJMPD..2744016P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PWW+19,
       author = {{Platts}, E. and {Weltman}, A. and {Walters}, A. and {Tendulkar}, S.~P. and
         {Gordin}, J.~E.~B. and {Kandhai}, S.},
        title = "{A living theory catalogue for fast radio bursts}",
      journal = {\physrep},
     keywords = {Fast radio bursts, Transients, Neutron stars, Black holes, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = aug,
       volume = {821},
        pages = {1-27},
          doi = {10.1016/j.physrep.2019.06.003},
archivePrefix = {arXiv},
       eprint = {1810.05836},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PhR...821....1P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dimoudi,
       author = {{Dimoudi}, Sofia and {Adamek}, Karel and {Thiagaraj}, Prabu and
         {Ransom}, Scott M. and {Karastergiou}, Aris and {Armour}, Wesley},
        title = "{A GPU Implementation of the Correlation Technique for Real-time Fourier Domain Pulsar Acceleration Searches}",
      journal = {\apjs},
     keywords = {instrumentation: miscellaneous, methods: data analysis, methods: numerical, pulsars: general, telescopes, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2018",
        month = "Dec",
       volume = {239},
       number = {2},
          eid = {28},
        pages = {28},
          doi = {10.3847/1538-4365/aabe88},
archivePrefix = {arXiv},
       eprint = {1804.05335},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJS..239...28D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INBOOK{Karel,
       author = {{Ad{\'a}mek}, Karel and {Armour}, Wesley},
        title = "{A GPU Implementation of the Harmonic Sum Algorithm}",
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
    booktitle = {Astronomical Data Analysis Software and Systems XXVII},
         year = "2019",
       editor = {{Teuben}, Peter J. and {Pound}, Marc W. and {Thomas}, Brian A. and
         {Warner}, Elizabeth M.},
       volume = {523},
       series = {Astronomical Society of the Pacific Conference Series},
        pages = {489},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ASPC..523..489A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Karel2,
       author = {{Ad{\'a}mek}, Karel and {Dimoudi}, Sofia and {Giles}, Mike and
         {Armour}, Wesley},
        title = "{Improved Acceleration of the GPU Fourier Domain Acceleration Search Algorithm}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2017",
        month = "Nov",
          eid = {arXiv:1711.10855},
        pages = {arXiv:1711.10855},
archivePrefix = {arXiv},
       eprint = {1711.10855},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017arXiv171110855A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Karel3,
       author = {{Ad{\'a}mek}, Karel and {Armour}, Wesley},
        title = "{A Real-time Single Pulse Detection Algorithm for GPUs}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2016",
        month = "Nov",
          eid = {arXiv:1611.09704},
        pages = {arXiv:1611.09704},
archivePrefix = {arXiv},
       eprint = {1611.09704},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016arXiv161109704A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DimoudiWesley,
       author = {{Dimoudi}, Sofia and {Armour}, Wesley},
        title = "{Pulsar Acceleration Searches on the GPU for the Square Kilometre Array}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2015",
        month = "Nov",
          eid = {arXiv:1511.07343},
        pages = {arXiv:1511.07343},
archivePrefix = {arXiv},
       eprint = {1511.07343},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015arXiv151107343D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LRL+16,
       author = {{Liu}, Tong and {Romero}, Gustavo E. and {Liu}, Mo-Lin and {Li}, Ang},
        title = "{Fast Radio Bursts and Their Gamma-Ray or Radio Afterglows as Kerr-Newman Black Hole Binaries}",
      journal = {\apj},
     keywords = {binaries: general, black hole physics, gamma-ray burst: general, gravitational waves, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = jul,
       volume = {826},
       number = {1},
          eid = {82},
        pages = {82},
          doi = {10.3847/0004-637X/826/1/82},
archivePrefix = {arXiv},
       eprint = {1602.06907},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...826...82L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Beloborodov,
       author = {{Beloborodov}, Andrei M.},
        title = "{A Flaring Magnetar in FRB 121102?}",
      journal = {\apjl},
     keywords = {dense matter, magnetic fields, radiation mechanisms: general, relativistic processes, stars: magnetars, supernovae: general, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = jul,
       volume = {843},
       number = {2},
          eid = {L26},
        pages = {L26},
          doi = {10.3847/2041-8213/aa78f3},
archivePrefix = {arXiv},
       eprint = {1702.08644},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...843L..26B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{MMS19,
       author = {{Metzger}, Brian D. and {Margalit}, Ben and {Sironi}, Lorenzo},
        title = "{Fast radio bursts as synchrotron maser emission from decelerating relativistic blast waves}",
      journal = {\mnras},
     keywords = {Shock waves, stars: neutron, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = may,
       volume = {485},
       number = {3},
        pages = {4091-4106},
          doi = {10.1093/mnras/stz700},
archivePrefix = {arXiv},
       eprint = {1902.01866},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.485.4091M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{CF12,
   author = {{Chandra}, P. and {Frail}, D.~A.},
    title = "{A Radio-selected Sample of Gamma-Ray Burst Afterglows}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1110.4124},
 keywords = {cosmology: observations, gamma-ray burst: general, hydrodynamics, radio continuum: general},
     year = 2012,
    month = feb,
   volume = 746,
      eid = {156},
    pages = {156},
      doi = {10.1088/0004-637X/746/2/156},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012ApJ...746..156C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DWY17,
       author = {{Dai}, Z.~G. and {Wang}, J.~S. and {Yu}, Y.~W.},
        title = "{Radio Emission from Pulsar Wind Nebulae without Surrounding Supernova Ejecta: Application to FRB 121102}",
      journal = {\apjl},
     keywords = {pulsars: general, radiation mechanisms: non-thermal, radio continuum: general, stars: neutron, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = mar,
       volume = {838},
       number = {1},
          eid = {L7},
        pages = {L7},
          doi = {10.3847/2041-8213/aa6745},
archivePrefix = {arXiv},
       eprint = {1702.05831},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...838L...7D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{RVI20,
       author = {{Resmi}, L and {Vink}, J and {Ishwara-Chandra}, C H},
        title = "{Implications of the lowest frequency detection of the persistent counterpart of FRB121102}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = oct,
          eid = {arXiv:2010.14334},
        pages = {arXiv:2010.14334},
archivePrefix = {arXiv},
       eprint = {2010.14334},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201014334R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{MBM19,
       author = {{Margalit}, Ben and {Berger}, Edo and {Metzger}, Brian D.},
        title = "{Fast Radio Bursts from Magnetars Born in Binary Neutron Star Mergers and Accretion Induced Collapse}",
      journal = {\apj},
     keywords = {Radio bursts, Magnetars, Gamma-ray bursts, Gravitational waves, 1339, 992, 629, 678, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = dec,
       volume = {886},
       number = {2},
          eid = {110},
        pages = {110},
          doi = {10.3847/1538-4357/ab4c31},
archivePrefix = {arXiv},
       eprint = {1907.00016},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...886..110M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{VRB+17,
       author = {{Vieyro}, F.~L. and {Romero}, G.~E. and {Bosch-Ramon}, V. and
         {Marcote}, B. and {del Valle}, M.~V.},
        title = "{A model for the repeating FRB 121102 in the AGN scenario}",
      journal = {\aap},
     keywords = {radio continuum: general, galaxies: dwarf, galaxies: jets, radiation mechanisms: non-thermal, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = jun,
       volume = {602},
          eid = {A64},
        pages = {A64},
          doi = {10.1051/0004-6361/201730556},
archivePrefix = {arXiv},
       eprint = {1704.08097},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...602A..64V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Zhang18,
       author = {{Zhang}, Bing},
        title = "{FRB 121102: A Repeatedly Combed Neutron Star by a Nearby Low-luminosity Accreting Supermassive Black Hole}",
      journal = {\apjl},
     keywords = {pulsars: general, radiation mechanisms: non-thermal, radio continuum: general, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = feb,
       volume = {854},
       number = {2},
          eid = {L21},
        pages = {L21},
          doi = {10.3847/2041-8213/aaadba},
archivePrefix = {arXiv},
       eprint = {1801.05436},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...854L..21Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{KIM13,
       author = {{Kashiyama}, Kazumi and {Ioka}, Kunihito and {M{\'e}sz{\'a}ros}, Peter},
        title = "{Cosmological Fast Radio Bursts from Binary White Dwarf Mergers}",
      journal = {\apjl},
     keywords = {binaries: general, radio continuum: general, white dwarfs, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = oct,
       volume = {776},
       number = {2},
          eid = {L39},
        pages = {L39},
          doi = {10.1088/2041-8205/776/2/L39},
archivePrefix = {arXiv},
       eprint = {1307.7708},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...776L..39K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PP13,
       author = {{Popov}, S.~B. and {Postnov}, K.~A.},
        title = "{Millisecond extragalactic radio bursts as magnetar flares}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = jul,
          eid = {arXiv:1307.4924},
        pages = {arXiv:1307.4924},
archivePrefix = {arXiv},
       eprint = {1307.4924},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013arXiv1307.4924P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{PP+16,
       author = {{Popov}, S.~B. and {Pshirkov}, M.~S.},
        title = "{Fast radio bursts counterparts in the scenario of supergiant pulses}",
      journal = {\mnras},
     keywords = {pulsars: general, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = oct,
       volume = {462},
       number = {1},
        pages = {L16-L20},
          doi = {10.1093/mnrasl/slw118},
archivePrefix = {arXiv},
       eprint = {1605.01992},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.462L..16P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998AJ....115.1693C,
       author = {{Condon}, J.~J. and {Cotton}, W.~D. and {Greisen}, E.~W. and {Yin}, Q.~F. and {Perley}, R.~A. and {Taylor}, G.~B. and {Broderick}, J.~J.},
        title = "{The NRAO VLA Sky Survey}",
      journal = {\aj},
     keywords = {CATALOGS, METHODS: DATA ANALYSIS, METHODS: OBSERVATIONAL, RADIO CONTINUUM, SURVEYS},
         year = 1998,
        month = may,
       volume = {115},
       number = {5},
        pages = {1693-1716},
          doi = {10.1086/300337},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998AJ....115.1693C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@MISC{2015ascl.soft02007M,
       author = {{Mohan}, Niruj and {Rafferty}, David},
        title = "{PyBDSF: Python Blob Detection and Source Finder}",
     keywords = {Software},
         year = 2015,
        month = feb,
          eid = {ascl:1502.007},
        pages = {ascl:1502.007},
archivePrefix = {ascl},
       eprint = {1502.007},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ascl.soft02007M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{CW+16,
       author = {{Cordes}, J.~M. and {Wasserman}, Ira},
        title = "{Supergiant pulses from extragalactic neutron stars}",
      journal = {\mnras},
     keywords = {gravitational lensing: micro, relativistic processes, stars: neutron, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = mar,
       volume = {457},
       number = {1},
        pages = {232-257},
          doi = {10.1093/mnras/stv2948},
archivePrefix = {arXiv},
       eprint = {1501.00753},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.457..232C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Totani13,
       author = {{Totani}, Tomonori},
        title = "{Cosmological Fast Radio Bursts from Binary Neutron Star Mergers}",
      journal = {\pasj},
     keywords = {gravitational waves, radio continuum: general, stars: binaries: general, stars: neutron, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = oct,
       volume = {65},
          eid = {L12},
        pages = {L12},
          doi = {10.1093/pasj/65.5.L12},
archivePrefix = {arXiv},
       eprint = {1307.4985},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013PASJ...65L..12T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BTA+17,
       author = {{Bassa}, C.~G. and {Tendulkar}, S.~P. and {Adams}, E.~A.~K. and
         {Maddox}, N. and {Bogdanov}, S. and {Bower}, G.~C. and
         {Burke-Spolaor}, S. and {Butler}, B.~J. and {Chatterjee}, S. and
         {Cordes}, J.~M. and {Hessels}, J.~W.~T. and {Kaspi}, V.~M. and
         {Law}, C.~J. and {Marcote}, B. and {Paragi}, Z. and {Ransom}, S.~M. and
         {Scholz}, P. and {Spitler}, L.~G. and {van Langevelde}, H.~J.},
        title = "{FRB 121102 Is Coincident with a Star-forming Region in Its Host Galaxy}",
      journal = {\apjl},
     keywords = {galaxies: dwarf, galaxies: star formation, gamma-ray burst: general, supernovae: general, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = jul,
       volume = {843},
       number = {1},
          eid = {L8},
        pages = {L8},
          doi = {10.3847/2041-8213/aa7a0c},
archivePrefix = {arXiv},
       eprint = {1705.07698},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...843L...8B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{CF12,
   author = {{Chandra}, P. and {Frail}, D.~A.},
    title = "{A Radio-selected Sample of Gamma-Ray Burst Afterglows}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1110.4124},
 keywords = {cosmology: observations, gamma-ray burst: general, hydrodynamics, radio continuum: general},
     year = 2012,
    month = feb,
   volume = 746,
      eid = {156},
    pages = {156},
      doi = {10.1088/0004-637X/746/2/156},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012ApJ...746..156C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SMB+18,
   author = {R.~M. {Shannon} et al},
    title = "{The dispersion-brightness relation for fast radio bursts from a wide-field survey}",
  journal = {\nat},
     year = 2018,
    month = oct,
   volume = 562,
    pages = {386-390},
      doi = {10.1038/s41586-018-0588-y},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2018Natur.562..386S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Swift_XRT,
       author = {{Burrows}, David N. and {Hill}, J.~E. and {Nousek}, J.~A. and
         {Kennea}, J.~A. and {Wells}, A. and {Osborne}, J.~P. and
         {Abbey}, A.~F. and {Beardmore}, A. and {Mukerjee}, K. and
         {Short}, A.~D.~T. and {Chincarini}, G. and {Campana}, S. and
         {Citterio}, O. and {Moretti}, A. and {Pagani}, C. and
         {Tagliaferri}, G. and {Giommi}, P. and {Capalbi}, M. and
         {Tamburelli}, F. and {Angelini}, L. and {Cusumano}, G. and
         {Br{\"a}uninger}, H.~W. and {Burkert}, W. and {Hartner}, G.~D.},
        title = "{The Swift X-Ray Telescope}",
      journal = {\ssr},
     keywords = {gamma-ray burst, X-ray telescope, Swift, X-ray instrumentation, X-ray CCD detector, X-ray mirrors, {\ensuremath{\gamma}}-ray burst, Astrophysics},
         year = 2005,
        month = oct,
       volume = {120},
       number = {3-4},
        pages = {165-195},
          doi = {10.1007/s11214-005-5097-2},
archivePrefix = {arXiv},
       eprint = {astro-ph/0508071},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005SSRv..120..165B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Swift_UVOT,
   title={The Swift Ultra-Violet/Optical Telescope},
   volume={120},
   ISSN={1572-9672},
   url={http://dx.doi.org/10.1007/s11214-005-5095-4},
   DOI={10.1007/s11214-005-5095-4},
   number={3-4},
   journal={Space Science Reviews},
   publisher={Springer Science and Business Media LLC},
   author={Roming, Peter W. A. and Kennedy, Thomas E. and Mason, Keith O. and Nousek, John A. and Ahr, Lindy and Bingham, Richard E. and Broos, Patrick S. and Carter, Mary J. and Hancock, Barry K. and Huckle, Howard E. and et al.},
   year={2005},
   month={Oct},
   pages={95–142}
}


@ARTICLE{HESS1U:2020,
       author = {{Ashton}, Terry and {Backes}, Michael and {Balzer}, Arnim and
         {Berge}, David and {Bolmont}, Julien and {Bonnefoy}, Simon and
         {Brun}, Francois and {Chaminade}, Thomas and {Delagnes}, Eric and
         {Fontaine}, Gerard and {F{\"u}{\ss}ling}, Matthias and
         {Giavitto}, Gianluca and {Giebels}, Berrie and
         {Glicenstein}, Jean-Francois and {Gr{\"a}ber}, Tobias and
         {Hinton}, Jim and {Jahnke}, Albert and {Klepser}, Stefan and
         {Kossatz}, Marko and {Kretzschmann}, Axel and {Lefranc}, Valentin and
         {Leich}, Holger and {Lenain}, Jean-Philippe and {L{\"u}decke}, Hartmut and
         {Lypova}, Iryna and {Manigot}, Pascal and {Marandon}, Vincent and
         {Moulin}, Emmanuel and {Murach}, Thomas and {de Naurois}, Mathieu and
         {Nayman}, Patrick and {Ohm}, Stefan and {Penno}, Marek and
         {Ross}, Duncan and {Salek}, David and {Schade}, Markus and
         {Schwab}, Thomas and {Shiningayamwe}, Kleopas and
         {Stegmann}, Christian and {Steppa}, Constantin and
         {Tavernet}, Jean-Paul and {Thornhill}, Julian and {Toussnel}, Francois and
         {Vincent}, Pascal},
        title = "{A NECTAr-based upgrade for the Cherenkov cameras of the H.E.S.S. 12-meter telescopes}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2020",
        month = "Jan",
          eid = {arXiv:2001.04510},
        pages = {arXiv:2001.04510},
archivePrefix = {arXiv},
       eprint = {2001.04510},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv200104510A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Aharonian2006a,
	Abstract = {Context: .The Crab nebula was observed with the HESS stereoscopic Cherenkov-telescope array between October 2003 and January 2005 for a total of 22.9 h (after data quality selection). This period of time partly overlapped with the commissioning phase of the experiment; observations were made with three operational telescopes in late 2003 and with the complete 4 telescope array in January-February 2004 and October 2004-January 2005.  Aims: .Observations of the Crab nebula are discussed and used as an example to detail the flux and spectral analysis procedures of HESS. The results are used to evaluate the systematic uncertainties in HESS flux measurements. Methods: .The Crab nebula data are analysed using standard HESS analysis procedures, which are described in detail. The flux and spectrum of gamma-rays from the source are calculated on run-by-run and monthly time-scales, and a correction is applied for long-term variations in the detector sensitivity. Comparisons of the measured flux and spectrum over the observation period, along with the results from a number of different analysis procedures are used to estimate systematic uncertainties in the measurements. Results: .The data, taken at a range of zenith angles between 45$\,^{\circ}$ and 65$\,^{\circ}$, show a clear signal with over 7500 excess events. The energy spectrum is found to follow a power law with an exponential cutoff, with photon index Gamma = 2.39 $\pm$ 0.03{stat} and cutoff energy Ec = (14.3 $\pm$ 2.1{stat}) TeV between 440 GeV and 40 TeV. The observed integral flux above 1 TeV is (2.26 $\pm$ 0.08{stat}) × 10-11 {cm-2 s-1}. The estimated systematic error on the flux measurement is estimated to be 20%, while the estimated systematic error on the spectral slope is 0.1.},
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...457..899A},
	Arxivurl = {http://arxiv.org/abs/astro-ph/0607333},
	Author = {{Aharonian}, F. and {Akhperjanian}, A.~G. and {Bazer-Bachi}, A.~R. and {Beilicke}, M. and {Benbow}, W. and {Berge}, D. and {Bernl{\"o}hr}, K. and {Boisson}, C. and {Bolz}, O. and {Borrel}, V. and {Braun}, I. and {Breitling}, F. and {Brown}, A.~M. and {B{\"u}hler}, R. and {B{\"u}sching}, I. and {Carrigan}, S. and {Chadwick}, P.~M. and {Chounet}, L.-M. and {Cornils}, R. and {Costamante}, L. and {Degrange}, B. and {Dickinson}, H.~J. and {Djannati-Ata{\"\i}}, A. and {O'C.~Drury}, L. and {Dubus}, G. and {Egberts}, K. and {Emmanoulopoulos}, D. and {Espigat}, P. and {Feinstein}, F. and {Ferrero}, E. and {Fiasson}, A. and {Fontaine}, G. and {Funk}, S. and {Funk}, S. and {Gallant}, Y.~A. and {Giebels}, B. and {Glicenstein}, J.~F. and {Goret}, P. and {Hadjichristidis}, C. and {Hauser}, D. and {Hauser}, M. and {Heinzelmann}, G. and {Henri}, G. and {Hermann}, G. and {Hinton}, J.~A. and {Hofmann}, W. and {Holleran}, M. and {Horns}, D. and {Jacholkowska}, A. and {de Jager}, O.~C. and {Kh{\'e}lifi}, B. and {Komin}, N. and {Konopelko}, A. and {Kosack}, K. and {Latham}, I.~J. and {Le Gallou}, R. and {Lemi{\`e}re}, A. and {Lemoine-Goumard}, M. and {Lohse}, T. and {Martin}, J.~M. and {Martineau-Huynh}, O. and {Marcowith}, A. and {Masterson}, C. and {McComb}, T.~J.~L. and {de Naurois}, M. and {Nedbal}, D. and {Nolan}, S.~J. and {Noutsos}, A. and {Orford}, K.~J. and {Osborne}, J.~L. and {Ouchrif}, M. and {Panter}, M. and {Pelletier}, G. and {Pita}, S. and {P{\"u}hlhofer}, G. and {Punch}, M. and {Raubenheimer}, B.~C. and {Raue}, M. and {Rayner}, S.~M. and {Reimer}, A. and {Reimer}, O. and {Ripken}, J. and {Rob}, L. and {Rolland}, L. and {Rowell}, G. and {Sahakian}, V. and {Saug{\'e}}, L. and {Schlenker}, S. and {Schlickeiser}, R. and {Schwanke}, U. and {Sol}, H. and {Spangler}, D. and {Spanier}, F. and {Steenkamp}, R. and {Stegmann}, C. and {Superina}, G. and {Tavernet}, J.-P. and {Terrier}, R. and {Th{\'e}oret}, C.~G. and {Tluczykont}, M. and {van Eldik}, C. and {Vasileiadis}, G. and {Venter}, C. and {Vincent}, P. and {V{\"o}lk}, H.~J. and {Wagner}, S.~J. and {Ward}, M.},
	Date-Added = {2018-10-11 16:19:14 +0200},
	Date-Modified = {2018-10-11 16:19:15 +0200},
	Doi = {10.1051/0004-6361:20065351},
	Eprint = {astro-ph/0607333},
	Journal = {A\&A},
	Keywords = {gamma rays: observations, ISM: individual objects: Crab, nebula, ISM: supernova remnants},
	Month = oct,
	Pages = {899-915},
	Title = {{Observations of the Crab nebula with HESS}},
	Volume = 457,
	Year = 2006
}

@ARTICLE{Heintz,
       author = {{Heintz}, Kasper E. and {Prochaska}, J. Xavier and {Simha}, Sunil and {Platts}, Emma and {Fong}, Wen-fai and {Tejos}, Nicolas and {Ryder}, Stuart D. and {Aggerwal}, Kshitij and {Bhandari}, Shivani and {Day}, Cherie K. and {Deller}, Adam T. and {Kilpatrick}, Charles D. and {Law}, Casey J. and {Macquart}, Jean-Pierre and {Mannings}, Alexandra and {Marnoch}, Lachlan J. and {Sadler}, Elaine M. and {Shannon}, Ryan M.},
        title = "{Host Galaxy Properties and Offset Distributions of Fast Radio Bursts: Implications for Their Progenitors}",
      journal = {\apj},
     keywords = {Galaxies, Interstellar medium, Star formation, Extragalactic radio sources, Radio bursts, Magnetars, 573, 847, 1569, 508, 1339, 992, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = nov,
       volume = {903},
       number = {2},
          eid = {152},
        pages = {152},
          doi = {10.3847/1538-4357/abb6fb},
archivePrefix = {arXiv},
       eprint = {2009.10747},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...903..152H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ravi19,
       author = {{Ravi}, Vikram},
        title = "{The prevalence of repeating fast radio bursts}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = jul,
       volume = {3},
        pages = {928-931},
          doi = {10.1038/s41550-019-0831-y},
archivePrefix = {arXiv},
       eprint = {1907.06619},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019NatAs...3..928R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

	
@article{RingBg,
   author = {{Berge}, D. and {Funk}, S. and {Hinton}, J.},
    title = "{Background modelling in very-high-energy {$\gamma$}-ray astronomy}",
  journal = {\aap},
   eprint = {astro-ph/0610959},
 keywords = {gamma rays: observations, methods: data analysis},
     year = 2007,
    month = may,
   volume = 466,
    pages = {1219-1229},
      doi = {10.1051/0004-6361:20066674},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...466.1219B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{de-Naurois2009a,
	Abstract = {We present a sophisticated gamma-ray likelihood reconstruction technique for imaging atmospheric Cerenkov telescopes. The technique is based on the comparison of the raw Cherenkov camera pixel images of a photon induced atmospheric particle shower with the predictions from a semi-analytical model. The approach was initiated by the CAT experiment in the 1990s, and has been further developed by a new fit algorithm based on a log-likelihood minimisation using all pixels in the camera, a precise treatment of night sky background noise, the use of stereoscopy and the introduction of first interaction depth as parameter of the model. The reconstruction technique provides a more precise direction and energy reconstruction of the photon induced shower compared to other techniques in use, together with a better gamma efficiency, especially at low energies, as well as an improved background rejection. For data taken with the H.E.S.S. experiment, the reconstruction technique yielded a factor of ˜2 better sensitivity compared to the H.E.S.S. standard reconstruction techniques based on second moments of the camera images (Hillas parameter technique).},
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009APh....32..231D},
	Archiveprefix = {arXiv},
	Arxivurl = {http://arxiv.org/abs/0907.2610},
	Author = {{de Naurois}, M. and {Rolland}, L.},
	Date-Added = {2018-10-11 16:27:16 +0200},
	Date-Modified = {2018-10-11 16:27:16 +0200},
	Doi = {10.1016/j.astropartphys.2009.09.001},
	Eprint = {0907.2610},
	Journal = {Astroparticle Physics},
	Month = dec,
	Pages = {231-252},
	Primaryclass = {astro-ph.IM},
	Title = {{A high performance likelihood reconstruction of {$\gamma$}-rays for imaging atmospheric Cherenkov telescopes}},
	Volume = 32,
	Year = 2009
	}

@article{Parsons2014a,
	Abstract = {We present a high-performance event reconstruction algorithm: an Image Pixel-wise fit for Atmospheric Cherenkov Telescopes (ImPACT). The reconstruction algorithm is based around the likelihood fitting of camera pixel amplitudes to an expected image template. A maximum likelihood fit is performed to find the best-fit shower parameters. A related reconstruction algorithm has already been shown to provide significant improvements over traditional reconstruction for both the CAT and H.E.S.S. experiments. We demonstrate a significant improvement to the template generation step of the procedure, by the use of a full Monte Carlo air shower simulation in combination with a ray-tracing optics simulation to more accurately model the expected camera images. This reconstruction step is combined with an MVA-based background rejection.},
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014APh....56...26P},
	Archiveprefix = {arXiv},
	Arxivurl = {http://arxiv.org/abs/1403.2993},
	Author = {{Parsons}, R.~D. and {Hinton}, J.~A.},
	Date-Added = {2018-10-11 16:32:40 +0200},
	Date-Modified = {2018-10-11 16:32:43 +0200},
	Doi = {10.1016/j.astropartphys.2014.03.002},
	Eprint = {1403.2993},
	Journal = {Astroparticle Physics},
	Month = apr,
	Pages = {26-34},
	Primaryclass = {astro-ph.IM},
	Title = {{A Monte Carlo template based analysis for air-Cherenkov arrays}},
	Volume = 56,
	Year = 2014
}
	
	
@article{HESS2_CAMERA2014,
   title={The camera of the fifth H.E.S.S. telescope. Part I: System description},
   volume={761},
   ISSN={0168-9002},
   url={http://dx.doi.org/10.1016/j.nima.2014.05.093},
   DOI={10.1016/j.nima.2014.05.093},
   journal={Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
   publisher={Elsevier BV},
   author={Bolmont, J. and Corona, P. and Gauron, P. and Ghislain, P. and Goffin, C. and Guevara Riveros, L. and Huppert, J.-F. and Martineau-Huynh, O. and Nayman, P. and Parraud, J.-M. and et al.},
   year={2014},
   month={Oct},
   pages={46–57}
}


@article{Rolke2005a,
	Abstract = {We study the frequentist properties of confidence intervals computed by the method known to statisticians as the Profile Likelihood. It is seen that the coverage of these intervals is surprisingly good over a wide range of possible parameter values for important classes of problems, in particular whenever there are additional nuisance parameters with statistical or systematic errors. Programs are available for calculating these intervals.},
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005NIMPA.551..493R},
	Author = {{Rolke}, W.~A. and {L{\'o}pez}, A.~M. and {Conrad}, J.},
	Date-Added = {2018-10-12 08:01:35 +0200},
	Date-Modified = {2018-10-12 08:01:35 +0200},
	Doi = {10.1016/j.nima.2005.05.068},
	Eprint = {physics/0403059},
	Journal = {Nuclear Instruments and Methods in Physics Research A},
	Month = oct,
	Pages = {493-503},
	Title = {{Limits and confidence intervals in the presence of nuisance parameters}},
	Volume = 551,
	Year = 2005
}

@article{UVOT_conversion_factor,
    author = {Poole, T. S. and Breeveld, A. A. and Page, M. J. and Landsman, W. and Holland, S. T. and Roming, P. and Kuin, N. P. M. and Brown, P. J. and Gronwall, C. and Hunsberger, S. and Koch, S. and Mason, K. O. and Schady, P. and Berk, D. Vanden and Blustin, A. J. and Boyd, P. and Broos, P. and Carter, M. and Chester, M. M. and Cucchiara, A. and Hancock, B. and Huckle, H. and Immler, S. and Ivanushkina, M. and Kennedy, T. and Marshall, F. and Morgan, A. and Pandey, S. B. and De Pasquale, M. and Smith, P. J. and Still, M.},
    title = "{Photometric calibration of the Swift ultraviolet/optical telescope}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {383},
    number = {2},
    pages = {627-645},
    year = {2007},
    month = {12},
    abstract = "{We present the photometric calibration of the Swift Ultraviolet/Optical Telescope (UVOT) which includes: optimum photometric and background apertures, effective area curves, colour transformations, conversion factors for count rates to flux and the photometric zero-points (which are accurate to better than 4 per cent) for each of the seven UVOT broad-band filters. The calibration was performed with observations of standard stars and standard star fields that represent a wide range of spectral star types. The calibration results include the position-dependent uniformity, and instrument response over the 1600–8000 Å operational range. Because the UVOT is a photon-counting instrument, we also discuss the effect of coincidence loss on the calibration results. We provide practical guidelines for using the calibration in UVOT data analysis. The results presented here supersede previous calibration results.}",
    issn = {0035-8711},
    doi = {10.1111/j.1365-2966.2007.12563.x},
    url = {https://doi.org/10.1111/j.1365-2966.2007.12563.x},
    eprint = {https://academic.oup.com/mnras/article-pdf/383/2/627/18572262/mnras0383-0627.pdf},
}



@INPROCEEDINGS{2016mks..confE...1J,
       author = {{Jonas}, J. and {MeerKAT Team}},
        title = "{The MeerKAT Radio Telescope}",
    booktitle = {MeerKAT Science: On the Pathway to the SKA},
         year = 2016,
        month = jan,
          eid = {1},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016mks..confE...1J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020ApJ...888...61M,
       author = {{Mauch}, T. and {Cotton}, W.~D. and {Condon}, J.~J. and
         {Matthews}, A.~M. and {Abbott}, T.~D. and {Adam}, R.~M. and
         {Aldera}, M.~A. and {Asad}, K.~M.~B. and {Bauermeister}, E.~F. and
         {Bennett}, T.~G.~H. and {Bester}, H. and {Botha}, D.~H. and
         {Brederode}, L.~R.~S. and {Brits}, Z.~B. and {Buchner}, S.~J. and
         {Burger}, J.~P. and {Camilo}, F. and {Chalmers}, J.~M. and
         {Cheetham}, T. and {de Villiers}, D. and {de Villiers}, M.~S. and
         {Dikgale-Mahlakoana}, M.~A. and {du Toit}, L.~J. and
         {Esterhuyse}, S.~W.~P. and {Fadana}, G. and {Fanaroff}, B.~L. and
         {Fataar}, S. and {February}, S. and {Frank}, B.~S. and
         {Gamatham}, R.~R.~G. and {Geyer}, M. and {Goedhart}, S. and
         {Gounden}, S. and {Gumede}, S.~C. and {Heywood}, I. and
         {Hlakola}, M.~J. and {Horrell}, J.~M.~G. and {Hugo}, B. and
         {Isaacson}, A.~R. and {J{\'o}zsa}, G.~I.~G. and {Jonas}, J.~L. and
         {Julie}, R.~P.~M. and {Kapp}, F.~B. and {Kasper}, V.~A. and
         {Kenyon}, J.~S. and {Kotz{\'e}}, P.~P.~A. and {Kriek}, N. and
         {Kriel}, H. and {Kusel}, T.~W. and {Lehmensiek}, R. and {Loots}, A. and
         {Lord}, R.~T. and {Lunsky}, B.~M. and {Madisa}, K. and {Magnus}, L.~G. and
         {Main}, J.~P.~L. and {Malan}, J.~A. and {Manley}, J.~R. and
         {Marais}, S.~J. and {Martens}, A. and {Merry}, B. and {Millenaar}, R. and
         {Mnyandu}, N. and {Moeng}, I.~P.~T. and {Mokone}, O.~J. and
         {Monama}, T.~E. and {Mphego}, M.~C. and {New}, W.~S. and
         {Ngcebetsha}, B. and {Ngoasheng}, K.~J. and {Ockards}, M.~T.~O. and
         {Oozeer}, N. and {Otto}, A.~J. and {Patel}, A.~A. and
         {Peens-Hough}, A. and {Perkins}, S.~J. and {Ramaila}, A.~J.~T. and
         {Ramudzuli}, Z.~R. and {Renil}, R. and {Richter}, L.~L. and
         {Robyntjies}, A. and {Salie}, S. and {Schollar}, C.~T.~G. and
         {Schwardt}, L.~C. and {Serylak}, M. and {Siebrits}, R. and
         {Sirothia}, S.~K. and {Smirnov}, O.~M. and {Sofeya}, L. and
         {Stone}, G. and {Taljaard}, B. and {Tasse}, C. and {Theron}, I.~P. and
         {Tiplady}, A.~J. and {Toruvanda}, O. and {Twum}, S.~N. and
         {van Balla}, T.~J. and {van der Byl}, A. and {van der Merwe}, C. and
         {Van Tonder}, V. and {Wallace}, B.~H. and {Welz}, M.~G. and
         {Williams}, L.~P. and {Xaia}, B.},
        title = "{The 1.28 GHz MeerKAT DEEP2 Image}",
      journal = {\apj},
     keywords = {Radio telescopes, Galaxy counts, Star formation, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = jan,
       volume = {888},
       number = {2},
          eid = {61},
        pages = {61},
          doi = {10.3847/1538-4357/ab5d2d},
archivePrefix = {arXiv},
       eprint = {1912.06212},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...888...61M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016JAI.....541001H,
       author = {{Hickish}, Jack and {Abdurashidova}, Zuhra and {Ali}, Zaki and
         {Buch}, Kaushal D. and {Chaudhari}, Sandeep C. and {Chen}, Hong and
         {Dexter}, Matthew and {Domagalski}, Rachel Simone and {Ford}, John and
         {Foster}, Griffin and {George}, David and {Greenberg}, Joe and
         {Greenhill}, Lincoln and {Isaacson}, Adam and {Jiang}, Homin and
         {Jones}, Glenn and {Kapp}, Francois and {Kriel}, Henno and
         {Lacasse}, Rich and {Lutomirski}, Andrew and {MacMahon}, David and
         {Manley}, Jason and {Martens}, Andrew and {McCullough}, Randy and
         {Muley}, Mekhala V. and {New}, Wesley and {Parsons}, Aaron and
         {Price}, Daniel C. and {Primiani}, Rurik A. and {Ray}, Jason and
         {Siemion}, Andrew and {van Tonder}, Verees{\'e} and
         {Vertatschitsch}, Laura and {Wagner}, Mark and {Weintroub}, Jonathan and
         {Werthimer}, Dan},
        title = "{A Decade of Developing Radio-Astronomy Instrumentation using CASPER Open-Source Technology}",
      journal = {Journal of Astronomical Instrumentation},
     keywords = {CASPER, digital signal processing, radio-astronomy, instrumentation, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2016,
        month = dec,
       volume = {5},
       number = {4},
          eid = {1641001-12},
        pages = {1641001-12},
          doi = {10.1142/S2251171716410014},
archivePrefix = {arXiv},
       eprint = {1611.01826},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016JAI.....541001H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012A&A...539A..95O,
       author = {{Offringa}, A.~R. and {van de Gronde}, J.~J. and {Roerdink}, J.~B.~T.~M.},
        title = "{A morphological algorithm for improving radio-frequency interference detection}",
      journal = {\aap},
     keywords = {instrumentation: interferometers, methods: data analysis, techniques: interferometric, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2012,
        month = mar,
       volume = {539},
          eid = {A95},
        pages = {A95},
          doi = {10.1051/0004-6361/201118497},
archivePrefix = {arXiv},
       eprint = {1201.3364},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...539A..95O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2007ASPC..376..127M,
       author = {{McMullin}, J.~P. and {Waters}, B. and {Schiebel}, D. and {Young}, W. and
         {Golap}, K.},
        title = "{CASA Architecture and Applications}",
    booktitle = {Astronomical Data Analysis Software and Systems XVI},
         year = 2007,
       editor = {{Shaw}, R.~A. and {Hill}, F. and {Bell}, D.~J.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {376},
        month = oct,
        pages = {127},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ASPC..376..127M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014MNRAS.444..606O,
       author = {{Offringa}, A.~R. and {McKinley}, B. and {Hurley-Walker}, N. and
         {Briggs}, F.~H. and {Wayth}, R.~B. and {Kaplan}, D.~L. and
         {Bell}, M.~E. and {Feng}, L. and {Neben}, A.~R. and {Hughes}, J.~D. and
         {Rhee}, J. and {Murphy}, T. and {Bhat}, N.~D.~R. and {Bernardi}, G. and
         {Bowman}, J.~D. and {Cappallo}, R.~J. and {Corey}, B.~E. and {Deshpand
        e}, A.~A. and {Emrich}, D. and {Ewall-Wice}, A. and {Gaensler}, B.~M. and
         {Goeke}, R. and {Greenhill}, L.~J. and {Hazelton}, B.~J. and
         {Hindson}, L. and {Johnston-Hollitt}, M. and {Jacobs}, D.~C. and
         {Kasper}, J.~C. and {Kratzenberg}, E. and {Lenc}, E. and
         {Lonsdale}, C.~J. and {Lynch}, M.~J. and {McWhirter}, S.~R. and
         {Mitchell}, D.~A. and {Morales}, M.~F. and {Morgan}, E. and
         {Kudryavtseva}, N. and {Oberoi}, D. and {Ord}, S.~M. and {Pindor}, B. and
         {Procopio}, P. and {Prabu}, T. and {Riding}, J. and {Roshi}, D.~A. and
         {Shankar}, N. Udaya and {Srivani}, K.~S. and {Subrahmanyan}, R. and
         {Tingay}, S.~J. and {Waterson}, M. and {Webster}, R.~L. and
         {Whitney}, A.~R. and {Williams}, A. and {Williams}, C.~L.},
        title = "{WSCLEAN: an implementation of a fast, generic wide-field imager for radio astronomy}",
      journal = {\mnras},
     keywords = {instrumentation: interferometers, methods: observational, techniques: interferometric, radio continuum: general, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2014,
        month = oct,
       volume = {444},
       number = {1},
        pages = {606-619},
          doi = {10.1093/mnras/stu1368},
archivePrefix = {arXiv},
       eprint = {1407.1943},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.444..606O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018MNRAS.478.2399K,
       author = {{Kenyon}, J.~S. and {Smirnov}, O.~M. and {Grobler}, T.~L. and
         {Perkins}, S.~J.},
        title = "{CUBICAL - fast radio interferometric calibration suite exploiting complex optimization}",
      journal = {\mnras},
     keywords = {instrumentation: interferometers, methods: analytical, methods: numerical, techniques: interferometric, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = aug,
       volume = {478},
       number = {2},
        pages = {2399-2415},
          doi = {10.1093/mnras/sty1221},
archivePrefix = {arXiv},
       eprint = {1805.03410},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.478.2399K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{uvot_psf,
    author = {Breeveld, A. A. and Curran, P. A. and Hoversten, E. A. and Koch, S. and Landsman, W. and Marshall, F. E. and Page, M. J. and Poole, T. S. and Roming, P. and Smith, P. J. and Still, M. and Yershov, V. and Blustin, A. J. and Brown, P. J. and Gronwall, C. and Holland, S. T. and Kuin, N. P. M. and McGowan, K. and Rosen, S. and Boyd, P. and Broos, P. and Carter, M. and Chester, M. M. and Hancock, B. and Huckle, H. and Immler, S. and Ivanushkina, M. and Kennedy, T. and Mason, K. O. and Morgan, A. N. and Oates, S. and De Pasquale, M. and Schady, P. and Siegel, M. and Vanden Berk, D.},
    title = "{Further calibration of the Swift ultraviolet/optical telescope}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {406},
    number = {3},
    pages = {1687-1700},
    year = {2010},
    month = {08},
    abstract = "{The Ultraviolet/Optical Telescope (UVOT) is one of three instruments onboard the Swift observatory. The photometric calibration has been published, and this paper follows up with details on other aspects of the calibration including a measurement of the point spread function with an assessment of the orbital variation and the effect on photometry. A correction for large-scale variations in sensitivity over the field of view is described, as well as a model of the coincidence loss which is used to assess the coincidence correction in extended regions. We have provided a correction for the detector distortion and measured the resulting internal astrometric accuracy of the UVOT, also giving the absolute accuracy with respect to the International Celestial Reference System. We have compiled statistics on the background count rates, and discuss the sources of the background, including instrumental scattered light. In each case, we describe any impact on UVOT measurements, whether any correction is applied in the standard pipeline data processing or whether further steps are recommended.}",
    issn = {0035-8711},
    doi = {10.1111/j.1365-2966.2010.16832.x},
    url = {https://doi.org/10.1111/j.1365-2966.2010.16832.x},
    eprint = {https://academic.oup.com/mnras/article-pdf/406/3/1687/2997075/mnras0406-1687.pdf},
}



@article{SDSS-DR12,
	doi = {10.1088/0067-0049/219/1/12},
	url = {https://doi.org/10.1088%2F0067-0049%2F219%2F1%2F12},
	year = 2015,
	month = {jul},
	publisher = {{IOP} Publishing},
	volume = {219},
	number = {1},
	pages = {12},
	author = {Shadab Alam and Franco D. Albareti and Carlos Allende Prieto and F. Anders and Scott F. Anderson and Timothy Anderton and Brett H. Andrews and Eric Armengaud and {\'{E}}ric Aubourg and Stephen Bailey and Sarbani Basu and Julian E. Bautista and Rachael L. Beaton and Timothy C. Beers and Chad F. Bender and Andreas A. Berlind and Florian Beutler and Vaishali Bhardwaj and Jonathan C. Bird and Dmitry Bizyaev and Cullen H. Blake and Michael R. Blanton and Michael Blomqvist and John J. Bochanski and Adam S. Bolton and Jo Bovy and A. Shelden Bradley and W. N. Brandt and D. E. Brauer and J. Brinkmann and Peter J. Brown and Joel R. Brownstein and Angela Burden and Etienne Burtin and Nicol{\'{a}}s G. Busca and Zheng Cai and Diego Capozzi and Aurelio Carnero Rosell and Michael A. Carr and Ricardo Carrera and K. C. Chambers and William James Chaplin and Yen-Chi Chen and Cristina Chiappini and S. Drew Chojnowski and Chia-Hsun Chuang and Nicolas Clerc and Johan Comparat and Kevin Covey and Rupert A. C. Croft and Antonio J. Cuesta and Katia Cunha and Luiz N. da Costa and Nicola Da Rio and James R. A. Davenport and Kyle S. Dawson and Nathan De Lee and Timoth{\'{e}}e Delubac and Rohit Deshpande and Saurav Dhital and Let{\'{\i}}cia Dutra-Ferreira and Tom Dwelly and Anne Ealet and Garrett L. Ebelke and Edward M. Edmondson and Daniel J. Eisenstein and Tristan Ellsworth and Yvonne Elsworth and Courtney R. Epstein and Michael Eracleous and Stephanie Escoffier and Massimiliano Esposito and Michael L. Evans and Xiaohui Fan and Emma Fern{\'{a}}ndez-Alvar and Diane Feuillet and Nurten Filiz Ak and Hayley Finley and Alexis Finoguenov and Kevin Flaherty and Scott W. Fleming and Andreu Font-Ribera and Jonathan Foster and Peter M. Frinchaboy and J. G. Galbraith-Frew and Rafael A. Garc{\'{\i}}a and D. A. Garc{\'{\i}}a-Hern{\'{a}}ndez and Ana E. Garc{\'{\i}}a P{\'{e}}rez and Patrick Gaulme and Jian Ge and R. G{\'{e}}nova-Santos and A. Georgakakis and Luan Ghezzi and Bruce A. Gillespie and L{\'{e}}o Girardi and Daniel Goddard and Satya Gontcho A Gontcho and Jonay I. Gonz{\'{a}}lez Hern{\'{a}}ndez and Eva K. Grebel and Paul J. Green and Jan Niklas Grieb and Nolan Grieves and James E. Gunn and Hong Guo and Paul Harding and Sten Hasselquist and Suzanne L. Hawley and Michael Hayden and Fred R. Hearty and Saskia Hekker and Shirley Ho and David W. Hogg and Kelly Holley-Bockelmann and Jon A. Holtzman and Klaus Honscheid and Daniel Huber and Joseph Huehnerhoff and Inese I. Ivans and Linhua Jiang and Jennifer A. Johnson and Karen Kinemuchi and David Kirkby and Francisco Kitaura and Mark A. Klaene and Gillian R. Knapp and Jean-Paul Kneib and Xavier P. Koenig and Charles R. Lam and Ting-Wen Lan and Dustin Lang and Pierre Laurent and Jean-Marc Le Goff and Alexie Leauthaud and Khee-Gan Lee and Young Sun Lee and Timothy C. Licquia and Jian Liu and Daniel C. Long and Mart{\'{\i}}n L{\'{o}}pez-Corredoira and Diego Lorenzo-Oliveira and Sara Lucatello and Britt Lundgren and Robert H. Lupton and Claude E. Mack III and Suvrath Mahadevan and Marcio A. G. Maia and Steven R. Majewski and Elena Malanushenko and Viktor Malanushenko and A. Manchado and Marc Manera and Qingqing Mao and Claudia Maraston and Robert C. Marchwinski and Daniel Margala and Sarah L. Martell and Marie Martig and Karen L. Masters and Savita Mathur and Cameron K. McBride and Peregrine M. McGehee and Ian D. McGreer and Richard G. McMahon and Brice M{\'{e}}nard and Marie-Luise Menzel and Andrea Merloni and Szabolcs M{\'{e}}sz{\'{a}}ros and Adam A. Miller and Jordi Miralda-Escud{\'{e}} and Hironao Miyatake and Antonio D. Montero-Dorta and Surhud More and Eric Morganson and Xan Morice-Atkinson and Heather L. Morrison and Beno{\^}it Mosser and Demitri Muna and Adam D. Myers and Kirpal Nandra and Jeffrey A. Newman and Mark Neyrinck and Duy Cuong Nguyen and Robert C. Nichol and David L. Nidever and Pasquier Noterdaeme and Sebasti{\'{a}}n E. Nuza and Julia E. O'Connell and Robert W. O'Connell and Ross O'Connell and Ricardo L. C. Ogando and Matthew D. Olmstead and Audrey E. Oravetz and Daniel J. Oravetz and Keisuke Osumi and Russell Owen and Deborah L. Padgett and Nikhil Padmanabhan and Martin Paegert and Nathalie Palanque-Delabrouille and Kaike Pan and John K. Parejko and Isabelle P{\^{a}}ris and Changbom Park and Petchara Pattarakijwanich and M. Pellejero-Ibanez and Joshua Pepper and Will J. Percival and Ismael P{\'{e}}rez-Fournon and Ignasi Pe{\textasciiacute}rez-Ra{\textasciigrave}fols and Patrick Petitjean and Matthew M. Pieri and Marc H. Pinsonneault and Gustavo F. Porto de Mello and Francisco Prada and Abhishek Prakash and Adrian M. Price-Whelan and Pavlos Protopapas and M. Jordan Raddick and Mubdi Rahman and Beth A. Reid and James Rich and Hans-Walter Rix and Annie C. Robin and Constance M. Rockosi and Tha{\'{\i}}se S. Rodrigues and Sergio Rodr{\'{\i}}guez-Torres and Natalie A. Roe and Ashley J. Ross and Nicholas P. Ross and Graziano Rossi and John J. Ruan and J. A. Rubi{\~{n}}o-Mart{\'{\i}}n and Eli S. Rykoff and Salvador Salazar-Albornoz and Mara Salvato and Lado Samushia and Ariel G. S{\'{a}}nchez and Bas{\'{\i}}lio Santiago and Conor Sayres and Ricardo P. Schiavon and David J. Schlegel and Sarah J. Schmidt and Donald P. Schneider and Mathias Schultheis and Axel D. Schwope and C. G. Sc{\'{o}}ccola and Caroline Scott and Kris Sellgren and Hee-Jong Seo and Aldo Serenelli and Neville Shane and Yue Shen and Matthew Shetrone and Yiping Shu and V. Silva Aguirre and Thirupathi Sivarani and M. F. Skrutskie and An{\v{z}}e Slosar and Verne V. Smith and Fl{\'{a}}via Sobreira and Diogo Souto and Keivan G. Stassun and Matthias Steinmetz and Dennis Stello and Michael A. Strauss and Alina Streblyanska and Nao Suzuki and Molly E. C. Swanson and Jonathan C. Tan and Jamie Tayar and Ryan C. Terrien and Aniruddha R. Thakar and Daniel Thomas and Neil Thomas and Benjamin A. Thompson and Jeremy L. Tinker and Rita Tojeiro and Nicholas W. Troup and Mariana Vargas-Maga{\~{n}}a and Jose A. Vazquez and Licia Verde and Matteo Viel and Nicole P. Vogt and David A. Wake and Ji Wang and Benjamin A. Weaver and David H. Weinberg and Benjamin J. Weiner and Martin White and John C. Wilson and John P. Wisniewski and W. M. Wood-Vasey and Christophe Ye{\textasciigrave}che and Donald G. York and Nadia L. Zakamska and O. Zamora and Gail Zasowski and Idit Zehavi and Gong-Bo Zhao and Zheng Zheng and Xu Zhou (周旭) and Zhimin Zhou (周志民) and Hu Zou (邹虎) and Guangtun Zhu},
	title = {{THE} {ELEVENTH} {AND} {TWELFTH} {DATA} {RELEASES} {OF} {THE} {SLOAN} {DIGITAL} {SKY} {SURVEY}: {FINAL} {DATA} {FROM} {SDSS}-{III}},
	journal = {The Astrophysical Journal Supplement Series},
	abstract = {The third generation of the Sloan Digital Sky Survey (SDSS-III) took data from 2008 to 2014 using the original SDSS wide-field imager, the original and an upgraded multi-object fiber-fed optical spectrograph, a new near-infrared high-resolution spectrograph, and a novel optical interferometer. All of the data from SDSS-III are now made public. In particular, this paper describes Data Release 11 (DR11) including all data acquired through 2013 July, and Data Release 12 (DR12) adding data acquired through 2014 July (including all data included in previous data releases), marking the end of SDSS-III observing. Relative to our previous public release (DR10), DR12 adds one million new spectra of galaxies and quasars from the Baryon Oscillation Spectroscopic Survey (BOSS) over an additional 3000 deg2 of sky, more than triples the number of H-band spectra of stars as part of the Apache Point Observatory (APO) Galactic Evolution Experiment (APOGEE), and includes repeated accurate radial velocity measurements of 5500 stars from the Multi-object APO Radial Velocity Exoplanet Large-area Survey (MARVELS). The APOGEE outputs now include the measured abundances of 15 different elements for each star. In total, SDSS-III added 5200 deg2 of ugriz imaging; 155,520 spectra of 138,099 stars as part of the Sloan Exploration of Galactic Understanding and Evolution 2 (SEGUE-2) survey; 2,497,484 BOSS spectra of 1,372,737 galaxies, 294,512 quasars, and 247,216 stars over 9376 deg2; 618,080 APOGEE spectra of 156,593 stars; and 197,040 MARVELS spectra of 5513 stars. Since its first light in 1998, SDSS has imaged over 1/3 of the Celestial sphere in five bands and obtained over five million astronomical spectra.}
}


@ARTICLE{XRT_CURVE_1,
       author = {{Evans}, P.~A. and {Beardmore}, A.~P. and {Page}, K.~L. and
         {Tyler}, L.~G. and {Osborne}, J.~P. and {Goad}, M.~R. and
         {O'Brien}, P.~T. and {Vetere}, L. and {Racusin}, J. and {Morris}, D. and
         {Burrows}, D.~N. and {Capalbi}, M. and {Perri}, M. and {Gehrels}, N. and
         {Romano}, P.},
        title = "{An online repository of Swift/XRT light curves of {\ensuremath{\gamma}}-ray bursts}",
      journal = {\aap},
     keywords = {gamma rays: bursts, gamma rays: observations, methods: data analysis, catalogs, Astrophysics},
         year = 2007,
        month = jul,
       volume = {469},
       number = {1},
        pages = {379-385},
          doi = {10.1051/0004-6361:20077530},
archivePrefix = {arXiv},
       eprint = {0704.0128},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007A&A...469..379E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{XRT_CURVE_2,
       author = {{Evans}, P.~A. and {Beardmore}, A.~P. and {Page}, K.~L. and
         {Osborne}, J.~P. and {O'Brien}, P.~T. and {Willingale}, R. and
         {Starling}, R.~L.~C. and {Burrows}, D.~N. and {Godet}, O. and
         {Vetere}, L. and {Racusin}, J. and {Goad}, M.~R. and {Wiersema}, K. and
         {Angelini}, L. and {Capalbi}, M. and {Chincarini}, G. and
         {Gehrels}, N. and {Kennea}, J.~A. and {Margutti}, R. and
         {Morris}, D.~C. and {Mountford}, C.~J. and {Pagani}, C. and
         {Perri}, M. and {Romano}, P. and {Tanvir}, N.},
        title = "{Methods and results of an automatic analysis of a complete sample of Swift-XRT observations of GRBs}",
      journal = {\mnras},
     keywords = {methods: data analysis, catalogues, gamma-rays: bursts, Astrophysics},
         year = 2009,
        month = aug,
       volume = {397},
       number = {3},
        pages = {1177-1201},
          doi = {10.1111/j.1365-2966.2009.14913.x},
archivePrefix = {arXiv},
       eprint = {0812.3662},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.397.1177E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{EBWB18,
       author = {{Eftekhari}, T. and {Berger}, E. and {Williams}, P.~K.~G. and {Blanchard}, P.~K.},
        title = "{Associating Fast Radio Bursts with Extragalactic Radio Sources: General Methodology and a Search for a Counterpart to FRB 170107}",
      journal = {\apj},
     keywords = {methods: statistical, radio continuum: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = jun,
       volume = {860},
       number = {1},
          eid = {73},
        pages = {73},
          doi = {10.3847/1538-4357/aac270},
archivePrefix = {arXiv},
       eprint = {1802.09525},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...860...73E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



%%% FRB20201124A ATels
@ARTICLE{WBG+21,
       author = {{Wharton}, Robert and {Bethapudi}, Suryarao and {Gautam}, Tasha and {Li}, Dongzi and {Lin}, Hsiu-Hsien and {Main}, Robert and {Marthi}, Viswesh and {Spitler}, Laura and {Pen}, Ue-Li},
        title = "{uGMRT detection of a persistent radio source coincident with FRB20201124A}",
      journal = {The Astronomer's Telegram},
     keywords = {Fast Radio Burst},
         year = 2021,
        month = apr,
       volume = {14529},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ATel14529....1W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{RPP+21,
       author = {{Ricci}, Roberto and {Piro}, Luigi and {Panessa}, Francesca and {O'Connor}, Brendan and {Lotti}, Simone and {Bruni}, Gabriele and {Zhang}, Bing},
        title = "{Detection of a persistent radio source at the location of FRB20201124A with VLA}",
      journal = {The Astronomer's Telegram},
     keywords = {Fast Radio Burst},
         year = 2021,
        month = apr,
       volume = {14549},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ATel14549....1R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{KFP+21,
       author = {{Kilpatrick}, C.~D. and {Fong}, W. and {Prochaska}, J.~X. and {Tejos}, N. and {Bhandari}, S. and {Day}, C.~K.},
        title = "{A redshift for the putative host galaxy of FRB20201124A}",
      journal = {The Astronomer's Telegram},
     keywords = {Fast Radio Burst},
         year = 2021,
        month = apr,
       volume = {14516},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ATel14516....1K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DBD+21,
       author = {{Day}, C.~K. and {Bhandari}, S. and {Deller}, A.~T. and {Shannon}, R.~M. and {Moss}, V.~A.},
        title = "{ASKAP localisation of the FRB 20201124A source}",
      journal = {The Astronomer's Telegram},
     keywords = {Fast Radio Burst},
         year = 2021,
        month = apr,
       volume = {14515},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ATel14515....1D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MKH+21,
       author = {{Marcote}, B. and {Kirsten}, F. and {Hessels}, J.~W.~T. and {Nimmo}, K. and {Keimpema}, A. and {Paragi}, Z. and {Bach}, U. and {Burgay}, M. and {Corongiu}, A. and {Feiler}, R. and {Forss{\'e}n}, O. and {Gawronski}, M. and {Giroletti}, M. and {Gopinath}, A. and {Hewitt}, D.~M. and {Karuppusamy}, R. and {Kramer}, M. and {Ould-Boukattine}, O.~S. and {Pilia}, M. and {Snelders}, M.~P. and {Spitler}, L. and {Surcis}, G. and {Trudu}, M. and {Yang}, J.},
        title = "{VLBI localization of FRB 20201124A and absence of persistent emission on milliarcsecond scales}",
      journal = {The Astronomer's Telegram},
     keywords = {Fast Radio Burst},
         year = 2021,
        month = may,
       volume = {14603},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ATel14603....1M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{KSF+21,
       author = {{Kumar}, P. and {Shannon}, R.~M. and {Flynn}, C. and {Os{\l}owski}, S. and {Bhandari}, S. and {Day}, C.~K. and {Deller}, A.~T. and {Farah}, W. and {Kaczmarek}, J.~F. and {Kerr}, M. and {Phillips}, C. and {Price}, D.~C. and {Qiu}, H. and {Thyagarajan}, N.},
        title = "{Extremely band-limited repetition from a fast radio burst source}",
      journal = {\mnras},
     keywords = {methods: data analysis, methods: observational, fast radio bursts, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = jan,
       volume = {500},
       number = {2},
        pages = {2525-2531},
          doi = {10.1093/mnras/staa3436},
archivePrefix = {arXiv},
       eprint = {2009.01214},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.500.2525K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{KSO+19,
       author = {{Kumar}, Pravir and {Shannon}, R.~M. and {Os{\l}owski}, Stefan and {Qiu}, Hao and {Bhandari}, Shivani and {Farah}, Wael and {Flynn}, Chris and {Kerr}, Matthew and {Lorimer}, D.~R. and {Macquart}, J. -P. and {Ng}, Cherry and {Phillips}, C.~J. and {Price}, Danny C. and {Spiewak}, Ren{\'e}e},
        title = "{Faint Repetitions from a Bright Fast Radio Burst Source}",
      journal = {\apjl},
     keywords = {Radio transient sources, Transient sources, 2008, 1851, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = dec,
       volume = {887},
       number = {2},
          eid = {L30},
        pages = {L30},
          doi = {10.3847/2041-8213/ab5b08},
archivePrefix = {arXiv},
       eprint = {1908.10026},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...887L..30K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{DDJ+21,
       author = {{Day}, Cherie K. and {Deller}, Adam T. and {James}, Clancy W. and {Lenc}, Emil and {Bhandari}, Shivani and {Shannon}, R.~M. and {Bannister}, Keith W.},
        title = "{Astrometric accuracy of snapshot fast radio burst localisations with ASKAP}",
      journal = {\pasa},
     keywords = {astrometry, fast radio bursts, radio interferometry, radio transient sources, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = jan,
       volume = {38},
          eid = {e050},
        pages = {e050},
          doi = {10.1017/pasa.2021.40},
archivePrefix = {arXiv},
       eprint = {2107.07068},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021PASA...38...50D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{CHIME/FRB+21,
       author = {{Chime/FRB Collaboration}},
        title = "{Recent high activity from a repeating Fast Radio Burst discovered by CHIME/FRB}",
      journal = {The Astronomer's Telegram},
     keywords = {Fast Radio Burst},
         year = 2021,
        month = mar,
       volume = {14497},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ATel14497....1C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LTC+21,
       author = {{Law}, Casey and {Tendulkar}, Shriharsh and {Clarke}, Tracy and {Aggarwal}, Kshitij and {Bethapudy}, Suryarao},
        title = "{VLA/realfast localization and deep imaging of FRB 20201124A}",
      journal = {The Astronomer's Telegram},
     keywords = {Fast Radio Burst},
         year = 2021,
        month = apr,
       volume = {14526},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ATel14526....1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{oxkat20,
       author = {{Heywood}, Ian},
        title = "{oxkat: Semi-automated imaging of MeerKAT observations}",
     keywords = {Software},
         year = 2020,
        month = sep,
          eid = {ascl:2009.003},
        pages = {ascl:2009.003},
archivePrefix = {ascl},
       eprint = {2009.003},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ascl.soft09003H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

 @article{hess_sgr1935,
  title={{Searching for TeV gamma-ray emission from SGR\,1935+2153 during its 2020 X-ray and radio active phase}},
  author="{H.E.S.S. collaboration}",
  year = {2021},
  journal = {ApJ},
  volume = {919},
  pages = {106},
  DOI = {10.3847/1538-4357/ac0fe1}
  }




@ARTICLE{li2020insighthxmt,
       author = {{Li}, C.~K. and {Lin}, L. and {Xiong}, S.~L. and {Ge}, M.~Y. and {Li}, X.~B. and {Li}, T.~P. and {Lu}, F.~J. and {Zhang}, S.~N. and {Tuo}, Y.~L. and {Nang}, Y. and {Zhang}, B. and {Xiao}, S. and {Chen}, Y. and {Song}, L.~M. and {Xu}, Y.~P. and {Liu}, C.~Z. and {Jia}, S.~M. and {Cao}, X.~L. and {Qu}, J.~L. and {Zhang}, S. and {Gu}, Y.~D. and {Liao}, J.~Y. and {Zhao}, X.~F. and {Tan}, Y. and {Nie}, J.~Y. and {Zhao}, H.~S. and {Zheng}, S.~J. and {Zheng}, Y.~G. and {Luo}, Q. and {Cai}, C. and {Li}, B. and {Xue}, W.~C. and {Bu}, Q.~C. and {Chang}, Z. and {Chen}, G. and {Chen}, L. and {Chen}, T.~X. and {Chen}, Y.~B. and {Chen}, Y.~P. and {Cui}, W. and {Cui}, W.~W. and {Deng}, J.~K. and {Dong}, Y.~W. and {Du}, Y.~Y. and {Fu}, M.~X. and {Gao}, G.~H. and {Gao}, H. and {Gao}, M. and {Gu}, Y.~D. and {Guan}, J. and {Guo}, C.~C. and {Han}, D.~W. and {Huang}, Y. and {Huo}, J. and {Jiang}, L.~H. and {Jiang}, W.~C. and {Jin}, J. and {Jin}, Y.~J. and {Kong}, L.~D. and {Li}, G. and {Li}, M.~S. and {Li}, W. and {Li}, X. and {Li}, X.~F. and {Li}, Y.~G. and {Li}, Z.~W. and {Liang}, X.~H. and {Liu}, B.~S. and {Liu}, G.~Q. and {Liu}, H.~W. and {Liu}, X.~J. and {Liu}, Y.~N. and {Lu}, B. and {Lu}, X.~F. and {Luo}, T. and {Ma}, X. and {Meng}, B. and {Ou}, G. and {Sai}, N. and {Shang}, R.~C. and {Song}, X.~Y. and {Sun}, L. and {Tao}, L. and {Wang}, C. and {Wang}, G.~F. and {Wang}, J. and {Wang}, W.~S. and {Wang}, Y.~S. and {Wen}, X.~Y. and {Wu}, B.~B. and {Wu}, B.~Y. and {Wu}, M. and {Xiao}, G.~C. and {Xu}, H. and {Yang}, J.~W. and {Yang}, S. and {Yang}, Y.~J. and {Yang}, Yi-Jung and {Yi}, Q.~B. and {Yin}, Q.~Q. and {You}, Y. and {Zhang}, A.~M. and {Zhang}, C.~M. and {Zhang}, F. and {Zhang}, H.~M. and {Zhang}, J. and {Zhang}, T. and {Zhang}, W. and {Zhang}, W.~C. and {Zhang}, W.~Z. and {Zhang}, Y. and {Zhang}, Yue and {Zhang}, Y.~F. and {Zhang}, Y.~J. and {Zhang}, Z. and {Zhang}, Zhi and {Zhang}, Z.~L. and {Zhou}, D.~K. and {Zhou}, J.~F. and {Zhu}, Y. and {Zhu}, Y.~X. and {Zhuang}, R.~L.},
        title = {HXMT identification of a non-thermal X-ray burst from SGR J1935+2154 and with FRB 200428},
      journal = {Nature Astronomy},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = feb,
          doi = {10.1038/s41550-021-01302-6},
archivePrefix = {arXiv},
       eprint = {2005.11071},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021NatAs.tmp...54L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Hu_2019,
   title={Opacities for photon splitting and pair creation in neutron star magnetospheres},
   volume={486},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1093/mnras/stz995},
   DOI={10.1093/mnras/stz995},
   number={3},
   journal={\mnras},
   publisher={Oxford University Press (OUP)},
   author={Hu, Kun and Baring, Matthew G and Wadiasingh, Zorawar and Harding, Alice K},
   year={2019},
   month={Apr},
   pages={3327–3349}
}


@ARTICLE{2016A&A...594A.116H,
       author = {{HI4PI Collaboration} and {Ben Bekhti}, N. and {Fl{\"o}er}, L. and {Keller}, R. and {Kerp}, J. and {Lenz}, D. and {Winkel}, B. and {Bailin}, J. and {Calabretta}, M.~R. and {Dedes}, L. and {Ford}, H.~A. and {Gibson}, B.~K. and {Haud}, U. and {Janowiecki}, S. and {Kalberla}, P.~M.~W. and {Lockman}, F.~J. and {McClure-Griffiths}, N.~M. and {Murphy}, T. and {Nakanishi}, H. and {Pisano}, D.~J. and {Staveley-Smith}, L.},
        title = "{HI4PI: A full-sky H I survey based on EBHIS and GASS}",
      journal = {\aap},
     keywords = {surveys, ISM: atoms, techniques: spectroscopic, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = oct,
       volume = {594},
          eid = {A116},
        pages = {A116},
          doi = {10.1051/0004-6361/201629178},
archivePrefix = {arXiv},
       eprint = {1610.06175},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...594A.116H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


